Ab initio calculations on nuclear matter properties including the effects of three-nucleons interaction

In this thesis, the ground state properties of nuclear matter, namely the energy per particle and the response to weak probes, are computed, studying the effects of three nucleon interactions. Both the variational approach, based on the formalism of correlated basis function, and the auxiliary field diffusion Monte Carlo method have been used. A scheme suitable to construct a density-dependent two-nucleon potential in correlated basis approach is discussed. The density dependent potential resulting from UIX three-nucleon force has been employed in auxiliary field diffusion Monte Carlo calculations that turned out to be in very good agreement with correlated basis variational results. Hence, the underbinding of symmetric nuclear matter has to be ascribed to deficiencies of the UXI potential. A comparative analysis of the equations of state of both pure neutron matter and symmetric nuclear matter obtained using a new generation of "chiral inspired" local three-body potentials has been performed. These potentials provide an excellent description of the properties of light nuclei, as well as of the neutron-deuteron doublet scattering length. The weak response of symmetric nuclear matter has been computed at three-body cluster level. Two-body effective interactions and one-body effective operators have been derived within the formalism of correlated basis functions. The inclusion of the three-body cluster term in the effective interaction allowed for a direct inclusion of the UIX three-nucleon potential. Moreover, the sizable unphysical dependence of the effective weak operator is removed once the three-body cluster term is taken into account.

==> app/linked.tex <==
To deal with fermions and to see how the cancellation of unlinked diagrams works, we start from a different definition of the $n$-body correlation function:
\begin{equation}
g_{n}(x_1,\dots,x_n)=
\frac{N!}{(N-n)!}\frac{1}{\rho^n}\,\frac
{\int dx_{n+1}\dots dx_N|\Psi^{0}_{MF}(X)|^2}{\int dx_1\dots dx_N|\Psi^{0}_{MF}(X)|^2}\, ,
\label{eq:def_corr_new}
\end{equation}
with $X$ indicating the whole spin/isospin and radial coordinates of the system. The corresponding MF $n$-body correlation function is defined analogously.

We now need a different definition of the MF one-body density matrix with respect to $l(i,j)$ defined in Eq. (\ref{eq:def_1bdm}). In order to do not make confusion, we denote this ``new'' MF one-body density matrix with $\rho(x_i,x_j)$. It is very useful in dealing with expectation values of spin/isospin dependent operators and it is defined by:
\begin{align}
\rho(x_i,x_j)&=\frac{1}{N}\sum_n \Psi_{n}^*(x_i)\Psi_{n}(x_j)\nonumber \\
&=\frac{1}{N}\sum_{|\mathbf{k}|<k_F}\phi_{\mathbf{k}_n}^*(\mathbf{r}_i)\phi_{\mathbf{k}_n}(\mathbf{r}_j)\sum_{a=1}^2\sum_{b=1}^2\chi^{*}_a(s_i)\chi_a(s_j)I^{*}_b(\tau_i)I^{*}_b(\tau_j)\nonumber \\
&=\frac{3}{4}\Big(\frac{\sin{y}-y\cos{y}}{y}\Big)\sum_{a=1}^2\sum_{b=1}^2\chi^{*}_a(s_i)\chi_a(s_j)I^{*}_b(\tau_i)I^{*}_b(\tau_j)\nonumber\\
&=\frac{3}{4}l(y)\sum_{a=1}^2\sum_{b=1}^2\chi^{*}_a(s_i)\chi_a(s_j)I^{*}_b(\tau_i)I^{*}_b(\tau_j)\, .
\end{align}
This result can be obtained in the same way of Eq. (\ref{eq:1bdm_fermi}), keeping in mind that $d=4$.
We now use another definition of the MF $n$-body correlation function, without computing the spin/isospin trace over all the particles:

Repeating the same passages which yielded Eq. (\ref{eq:num_last}), we find the numerator of $g_{2}(x_1,,x_2)$ to be:
\begin{align}
num &=\mathcal{N}f^2(\mathbf{r}_{12})\Big[g_{2}^{MF}(x_1,x_2)\nonumber \\
&+\sum_{n=3}^{N}\frac{\rho^{n-2}}{(n-2)!}\int dx_{3}\dots dx_n  X^{(n)}(x_1,x_2;x_3,x_4,\dots,x_n) g_{n}^{MF}(x_1,\dots,x_n)\Big]\, .
\label{eq:num_new}
\end{align}

What remains to compute is $g_{n}^{MF}(x_1,\dots,x_n)$ that gives rise to the exchange lines of the cluster diagrams.
We start from the easiest one:
\begin{equation}
g_{2}^{MF}(x_1,x_2)=\frac{N(N-1)}{\rho^2}\,\frac{\int dx_{3}\dots dx_N|\Psi^{0}_{MF}(X)|^2}{\int dx_1\dots dx_N|\Psi^{0}_{MF}(X)|^2}\,. 
\label{eq:def_radcorrMF_new}
\end{equation}
Also in this case we can express the modulus squared of $\Psi_{MF}$ in terms of the antisymmetrizing operator applied only to one side:
\begin{align}
\int dx_{3}\dots dx_N|\Psi^{0}_{MF}(X)|^2=&
\sqrt{2!}\frac{V^{N-2}}{N(N-1)}\,\sum_{n_i=1}^N \psi_{n_1}^*(x_1)\psi_{n_2}^*(x_2)\mathcal{A}[\psi_{n_1}(x_1)\psi_{n_2}(x_2)]=\nonumber \\
&\frac{V^{N-2}}{N(N-1)}[\rho(x_1,x_1)\rho(x_2,x_2)-\rho(x_1,x_2)\rho(x_2,x_1)]\, .
\end{align}
For the numerator of (\ref{eq:def_radcorrMF_new}) we get a factor $\Omega^N$, as in Eq. (\ref{eq:denomg_2}). Putting these two results in Eq. (\ref{eq:def_radcorrMF_new}) yields:
\begin{equation}
g_{2}^{MF}(x_1,x_2)=\rho(x_1,x_1)\rho(x_2,x_2)-\rho(x_1,x_2)\rho(x_2,x_1)\, .
\end{equation}
The above expression can be readily generalized to the case of the MF $n$-body correlation function, with the result:
\begin{equation}
g_{n}^{MF}(x_1,\dots,x_n)=\det|\rho(x_i,x_j)|\qquad i,j\in[1,n]\, .
\end{equation}
It is convenient to introduce a compact notation for the determinant:
\begin{equation}
\Delta_n(x_1,\dots,x_n)\equiv \det|\rho(x_i,x_j)|\qquad i,j\in[1,n]\, ,
\label{eq:def_Delta}
\end{equation}
so that:
\begin{equation}
g_{n}^{MF}(x_1,\dots,x_n)=\Delta_n(x_1,\dots,x_n)\, .
\end{equation}
If we replace $g_{n}^{MF}$ with $\Delta_n$ in Eq. (\ref{eq:num_new}) we get:
\begin{align}
num &=\mathcal{N}f^2(\mathbf{r}_{12})\Big[\Delta_2(x_1,x_2)\nonumber \\
&+\sum_{n=3}^{N}\frac{\rho^{n-2}}{(n-2)!}\int dx_{3}\dots dx_n  X^{(n)}(x_1,x_2;x_3,x_4,\dots,x_n) \Delta_{n}(x_1,\dots,x_n)\Big]\, .
\label{eq:num_last_new}
\end{align}
It may analogously be shown that the denominator of $g_{2}(x_1,,x_2)$ is:
\begin{align}
den &=\mathcal{N}\Big[1+\sum_{n=2}^{N}\frac{\rho^{n}}{n!}\int dx_{1}\dots dx_n  X^{(n)}(x_1,\dots,x_n) \Delta_{n}(x_1,\dots,x_n)\Big]\, .
\label{eq:den_new}
\end{align}
The diagrammatic rules are more or less the same we have already listed, but there are some differences. The various terms of the
determinants $\Delta_n$ are represented on the diagram by all the possible ways of drawing exchange lines. Now there are no more $1/d$
factors and each exchange line leaving the point $i$ and entering the point $j$ contributes the factor $\rho(x_i,x_j)$ to the diagram.
This is just a more general way of representing $g_{n}^{MF}$. 

By looking at the Eqs. (\ref{eq:num_last_new}) and (\ref{eq:den_new}), it seems that the problem of non exact cancellation of unlinked diagram is still there. This time we can use a trick. If we {\it define} $\Delta_n$ in terms of Eq. (\ref{eq:def_Delta}) for {\it any} value of $n$, but keeping $\mathbf{k}_F$ fixed, we find according to the theorem of Gram: 
\begin{equation}
\Delta_n=0\qquad \text{for}\quad p>N\, .
\end{equation}
Thus the sums in Eqs. (\ref{eq:num_last_new}) and (\ref{eq:den_new}) can be extended to infinity and now the cancellation of unlinked diagram is exact.  




==> app/ti.tex <==
By uniform systems, like nuclear matter, we mean homogenous and isotropic systems, characterized by translational and rotational invariance.  At this point it is worth to distinguish the radial part of the wave function, $\phi$, and the Pauli spinors describing the spin-isospin state of the nucleon, $\chi_{\sigma_i}$ and $\eta_{\tau_i}$
\begin{equation}
\psi(x)=\phi(\mathbf{r})\chi_{\sigma_i}\eta_{\tau_i}
\end{equation}

For the quantum mechanical point of view, translational invariance implies that the radial part of the translated wave function remains unchanged except for a phase factor
\begin{equation}
\phi(\mathbf{r}+\mathbf{a})=e^{if(\mathbf{a})}\phi(\mathbf{r})\, .
\label{eq:translation}
\end{equation}

The translation $\mathbf{r}\to \mathbf{r}+ c_1\, \mathbf{a}_1+c_2\,\mathbf{a}_2$ can be performed either all at once 
\begin{equation}
\phi(\mathbf{r}+ c_1\, \mathbf{a}_1+c_2\,\mathbf{a}_2)=e^{if(c_1\mathbf{a}_1+c_2\mathbf{a}_2)}\phi(\mathbf{r})\,
\end{equation}
or by translating $c_1$ times the wave function by the vector $\mathbf{a}_1$ and $c_2$ times by $\mathbf{a}_2$
\begin{equation}
\phi(\mathbf{r}+ c_1\, \mathbf{a}_1+c_2\,\mathbf{a}_2)=e^{ic_1f(\mathbf{a}_1)}e^{ic_2f(\mathbf{a}_2)}\phi(\mathbf{r})\,.
\end{equation}
Consequently, the phase has to be a linear function of the translation $\mathbf{a}$
\begin{equation}
f(\mathbf{a})=\mathbf{k}\cdot\mathbf{a}\, .
\end{equation}


Since differentiating $\phi(\mathbf{r}+\mathbf{a})$ with respect to $\mathbf{r}$ is equivalent to differentiating with respect to  $\mathbf{a}$, from Eq. (\ref{eq:translation}), one finds that $\psi(\mathbf{r})$ is an eigenvector of the translation operator
\begin{equation}
\vec{\nabla}\phi(\mathbf{r})=i[\vec{\nabla} f(\mathbf{a})]\phi(\mathbf{r})=i\mathbf{k}\phi(\mathbf{r})\,.
\end{equation}

The solution of the previous differential equation is a plane wave with wave vector $\mathbf{k}$
\begin{equation}
\phi(\mathbf{r})=\mathcal{N} e^{i\mathbf{k}\cdot\mathbf{r}}\, .
\end{equation}
where $\mathcal{N}$ is a normalization constant. {\color{red} It is worth noting that, despite an independent-particle picture of the quantum mechanical system is not always feasible and correlations are likely to be considered, the eigenfunctions of the hamiltonian are always eigenstates of the single particle momenta. This is indeed guaranteed by the translational symmetry of the system.}

==> tbp/prova.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5040.00,3770.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(946,984){\makebox(0,0)[r]{\strut{}$-0.8$}}%
      \put(946,1264){\makebox(0,0)[r]{\strut{}$-0.6$}}%
      \put(946,1544){\makebox(0,0)[r]{\strut{}$-0.4$}}%
      \put(946,1824){\makebox(0,0)[r]{\strut{}$-0.2$}}%
      \put(946,2105){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(946,2385){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \put(946,2665){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \put(946,2945){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \put(946,3225){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \put(946,3505){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(1741,484){\makebox(0,0){\strut{}$-2\pi$}}%
      \put(2301,484){\makebox(0,0){\strut{}$-\pi$}}%
      \put(2861,484){\makebox(0,0){\strut{}$0$}}%
      \put(3420,484){\makebox(0,0){\strut{}$\pi$}}%
      \put(3980,484){\makebox(0,0){\strut{}$2\pi$}}%
      \put(176,2104){\rotatebox{-270}{\makebox(0,0){\strut{}$y$}}}%
      \put(2860,154){\makebox(0,0){\strut{}$x$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3656,3332){\makebox(0,0)[r]{\strut{}$\sin(x)$}}%
    }%

